A Lockdown Perspective on the Hubble Tension (with comments from the SH0ES team)

This is a transcript of a talk that I gave in Cambridge on 17th July 2020 on the `Hubble tension'. I review the SH0ES analyses by Riess and collaborators and point out some internal inconsistencies, including a discrepancy between the relative distances inferred from Cepheids of two of the primary geometric distance anchors, the Large Magellanic Cloud (LMC) and NGC 4258. I then ask `what would it take to make SH0ES compatible with early time measurements?'. The answer is a systematic bias of 0.1 - 0.15 mag in the intercept of the Cepheid period-luminosity relations of SH0ES galaxies. Such a bias resolves the Hubble tension, the tension between the distance anchors, and the difference between SH0ES and the tip of the red giant branch (TRGB) distance ladder, as measured and calibrated by Freedman and collaborators. I show that the difference between the TRGB and SH0ES values of H0 is caused mainly by a systematic calibration offset. In the short term, observational efforts should be focussed on improving the calibrations of the distance anchors and nearby galaxies, rather than trying to measure distance moduli to more supernovae host galaxies. I argue that an independent distance estimate to NGC 4258 is particularly critical. With such observations, it should be possible, on a relatively short timescale, to establish definitively whether the Hubble tension really exists.

==> abstract.tex <==
This is a transcript of a talk that I gave in Cambridge on 17th July
2020 on the `Hubble tension'.  I review the SH0ES analyses by Riess
and collaborators and point out some internal inconsistencies,
including a discrepancy between the relative distances inferred from
Cepheids of two of the primary geometric distance anchors, the Large
Magellanic Cloud (LMC) and NGC 4258. I then ask `what would it take to
make SH0ES compatible with early time measurements?'. The answer is a
systematic bias of 0.1 - 0.15 mag in the intercept of the Cepheid
period-luminosity relations of SH0ES galaxies.  Such a bias resolves
the Hubble tension, the tension between the distance anchors, and the
difference between SH0ES and the tip of the red giant branch (TRGB)
distance ladder, as measured and calibrated by Freedman and
collaborators.  I show that the difference between the TRGB and SH0ES
values of H0 is caused mainly by a systematic calibration offset.  In
the short term, observational efforts should be focussed on improving
the calibrations of the distance anchors and nearby galaxies, rather
than trying to measure distance moduli to more supernovae host
galaxies. I argue that an independent distance estimate to NGC 4258 is
particularly critical. With such observations, it should be possible,
on a relatively short timescale, to establish definitively whether the
Hubble tension really exits. Includes responses from the SH0ES Team.

